NN-Defined Modulator: Reconfigurable and Portable Software Modulator on IoT Gateways

A physical-layer modulator is a vital component for an IoT gateway to map the symbols to signals. However, due to the soldered hardware chipsets on the gateway's motherboards or the diverse toolkits on different platforms for the software radio, the existing solutions either have limited extensibility or are platform-specific. Such limitation is hard to ignore when modulation schemes and hardware platforms have become extremely diverse. This paper presents a new paradigm of using neural networks as an abstraction layer for physical layer modulators in IoT gateway devices, referred to as NN-defined modulators. Our approach addresses the challenges of extensibility and portability for multiple technologies on various hardware platforms. The proposed NN-defined modulator uses a model-driven methodology rooted in solid mathematical foundations while having native support for hardware acceleration and portability to heterogeneous platforms. We conduct the evaluation of NN-defined modulators on different platforms, including Nvidia Jetson Nano and Raspberry Pi. Evaluations demonstrate that our NN-defined modulator effectively operates as conventional modulators and provides significant efficiency gains (up to $4.7\times$ on Nvidia Jetson Nano and $1.1\times$ on Raspberry Pi), indicating high portability. Furthermore, we show the real-world applications using our NN-defined modulators to generate ZigBee and WiFi packets, which are compliant with commodity TI CC2650 (ZigBee) and Intel AX201 (WiFi NIC), respectively.

==> Sections/3_Overview.tex <==
\section{System Overview}\label{sec:overview}

The architecture of the proposed Neural-Network-Defined (NN-defined) modulator is depicted in Figure~\ref{fig:deisgnoverview}. Firstly, there is a given modulator template rooted in solid mathematical foundations~(Section~\ref{sec:template}). Subsequently, a template can be configured in its parameters to implement specific modulation schemes either manually as in Section~\ref{sec:modulator}, or in a learning manner as in Section~\ref{sec:learning}. Next, the NN-defined modulator will be transformed into a unified NN framework capable of executing across heterogeneous platforms (Section~\ref{sec:portability}). The unified NN framework can be deployed onto various platforms and incorporated into the transmission pipeline (Section~\ref{sec:eval}).

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/Overview/DesignOverview.pdf}
    \vspace{-3mm} 
    \caption{Architecture of NN-defined modulator.}
    \label{fig:deisgnoverview}
    \vspace{-5mm} 
\end{figure}


==> Sections/TodoList.tex <==
\section{Todo}
Submission deadline: 5 May 11:59:59am
\begin{itemize}

{\color{red}
\item Applications in Motivation part. Perspective-1: reduce the development complexity for developer. \st{Perspective-2: reduce the deployment complexity for different platforms. Perspective-3: improve efficiency.} Finish before 4 May 14:00


\item \st{Introduce protocol-related design in design.}

\item \st{ ZigBee and WiFi applications in Evaluation. ZigBee diagram; WiFi diagram. WiFi data packet transmission.}}

\item \st{Refine the modulator schemes part. Add some diagrams to show the modulators of single carrier and Multicarrier. Finish before 4 May 16:00}

\item \st{Finish the related work/ Discussion/ Reference. Finish before 4 May 18:00}

\item Check format and typos. \st{Check the results in abstract and results in evaluation} Finish before 4 May 20:00

\item Font size in figures.

\item Final check.

\end{itemize}

